Solving the TTC 2011 Reengineering Case with Henshin

This paper presents the Henshin solution to the Model Transformations for Program Understanding case study as part of the Transformation Tool Contest 2011.

==> eptcsdata.tex <==
\providecommand{\firstpage}{181}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.17}{10.4204/EPTCS.74.17}}
\pdfoutput=1

